Compact representation for matrices of bounded twin-width

For every fixed $d \in \mathbb{N}$, we design a data structure that represents a binary $n \times n$ matrix that is $d$-twin-ordered. The data structure occupies $O_d(n)$ bits, which is the least one could hope for, and can be queried for entries of the matrix in time $O_d(\log \log n)$ per query.

==> prelims.tex <==
\section{Preliminaries}
In this section we introduce some basic definitions and knowledge related to twin-width. Twin-width is a new graph parameter first introduced in \cite{tww1}. One possible way to look at it is that it describes how much the graph is similar to a cograph. Cographs are precisely the graphs with twin-width $0$. There is a few alternative definitions of twin-width. Two of them are particularly interesting to us. The first one defines the twin-width of a graph via a contraction sequence associated with this graph. We recall this definition next, together with the related definition of a trigraph. %Throughout the entire paper a parameter $d$ is used, whose intuitive meaning is to bound the twin-width from above. 

\begin{definition}[after \cite{tww1}]
A \emph{trigraph} is a triple $(V,E,R)$, where $E,R \subseteq {{V}\choose {2}}$ and $E \cap R = \emptyset$. The set $E$ is referred to as edges, while the set $R$ is referred to as \emph{red edges}. A $d$-trigraph is a trigraph $(V,E,R)$, where $(V,R)$ has maximum degree bounded by $d$.   
\end{definition}

\begin{definition}[after \cite{tww1}]
Given a trigraph $\graphH=(V,E,R)$ and two vertices $u,v \in V$, we define the trigraph $\contraction{\graphH}{u}{v}=(V',E',R')$, where                                                                                 $V' = (V \setminus \{ u,v \}) \cup \{ w \} \text{ for some } w \notin V $ and
\begin{align*}                                                                                                     E' = \{ \{ x,y \} \in { {V'}\choose{2} } :&\{ x, y \} \in E \text{ and } \{x,y \} \cap \{u,v \} = \emptyset \text{ or } \\  
&x=w \text{ and } \{u,y \} \in E \text{ and } \{ v,y \} \in E \} \\
R' = \{ \{ x,y \} \in { {V'}\choose{2} }: &\{x,y \} \in R \text{ and } \{ x, y \} \cap \{u,v \} = \emptyset \text{ or }\\ &x=w \text{ and } \{u,y \} \in E \text{ and } \{ v,y \} \notin E  \text{ or }\\
 &x=w \text{ and } \{u,y \} \notin E \text{ and } \{ v,y \} \in E \text{ or } \\
 &x=w \text{ and } ( \{ u,y \} \in R \text{ or } \{ v,y \} \in R)
\}
\end{align*}
We refer to $\contraction{\graphH}{u}{v}$ as the contraction of $\graphH$. If both $\graphH$ and $\contraction{\graphH}{u}{v}$ are $d$-trigraphs then $\contraction{\graphH}{u}{v}$ is a $d$-contraction of $\graphH$.
\end{definition}

\begin{definition}
A graph $\graph=(V,E)$ on $n$ vertices is $d$-collapsible, if there exists a sequence of $d$-contractions $\graphH_n,\ldots,\graphH_1$, such that $\graphH_n=(V,E,\emptyset)$, $\graphH_{i-1}$ is a $d$-contraction of $\graphH_i$ for $i \in \interval{2}{n}$ and $\graphH_1$ is a singleton graph. We then refer to such contraction sequence as a $d$-sequence for $\graph$. 
\end{definition}

We are now ready to formally define the twin-width parameter.

\begin{definition}
The twin-width of $\graph$, denoted as $\tww{G}$, is minimum $d$ such that $\graph$ is $d$-collapsible. 
\end{definition}

The drawback of defining twin-width via $d$-sequence is that $d$-sequence is formally an object containing $n$ trigraphs, and thus quadratic in the size of the original graph. This can be circumvented. In \cite{tww3}, the authors define the \emph{ordered union tree} of a $d$-sequence, which is a tree decomposition for twin-width. We recall this definition after them.
\begin{definition}[after \cite{tww3}]\label{def:decomp}
The ordered union tree of a $d$-sequence $\graphH_n,\ldots,\graphH_1$ for a graph $\graph$ is a pair $(\tree,\arr)$ where $\tree$ is a rooted binary tree whose leaves are in one-to-one correspondence with $V(\graph)$, and $\arr$ is an array of length $n-1$ whose $i$-th entry is a pointer at a (distinct) internal node of $\tree$ representing the $i$-th contraction, i.e., whose rooted subtree has for leaves all the vertices of $\graph$ contained in the contracted vertex.
\end{definition}

The authors in \cite{tww3} claim, that for all considered graph classes of bounded twin-width, computing the ordered union tree is no harder than computing $d$-sequence.
Consider the ordered union tree $(\tree,\arr)$ of a $d$-sequence of a graph $\graph$. Traversing $\tree$ in a preorder fashion gives an order $<_{\tree,\arr}$ on vertices of $\graph$. According to  Definition~\ref{def:decomp}, each node of $\tree$ represents one contraction, and its rooted subtree has for leaves a subset of $V(G)$ which is an interval according to $<_{\tree,\arr}$. Thus, the $d$-sequence of $\graph$ can be represented as a sequence of intervals with endpoints in $\range{n}$. Observe as well, that 
swapping any two siblings in $\tree$ results in a different ordering of vertices of $G$, which also gives an interval representation of a $d$-sequence. This leads to the following two new definitions.

\begin{definition}
Let $(\tree,\arr)$ be an ordered union tree of a $d$-sequence of a $d$-collapsible graph $\graph$. An ordering $<_{\tree,\arr}$ orders $V(G)$ (leafs of $\tree$) according to the preorder traversal of $\tree$. An interval representation $\intrep{\tree}{\arr}$ is an ordered set of intervals $I_1,\ldots, I_{n-1}$, where $I_j=\interval{a_j}{b_j}$ is an interval in $\range{n}$, and $a_j$ and $b_j$ are the positions of the first and the last leaf (vertex of $\graph$) in the subtree of $\arr[j]$ according to $<_{\tree,\arr}$.   
\end{definition}

\begin{definition}
An ordering on a set of vertices $V$ of a $d$-collapsible graph $\graph$ is a twin-width ordering if it is a $<_{\tree,\arr}$ ordering for some ordered union tree $(\tree,\arr)$ of a $d$-sequence of $\graph$.   
\end{definition}

In \cite{tww3} the authors show, that given the ordered union tree for a $d$-sequence, one can compute a very nice and compact representation of $\graph$ called an interval biclique partition. We recall this representation now. 

\begin{definition}[after \cite{tww3}]\label{def:ibp}
An interval biclique partition (or $\ibp$, for short) of a graph $\graph$ on vertex set $\range{n}$ is a set
$\ibpset$ of bicliques that edge-partitions $\graph$ where each biclique $\bc{A}{B} \in \ibpset$ is such that both
sides $A$ and $B$ are two (disjoint) discrete intervals of $\range{n}$. 
\end{definition}

Every graph $\graph$ admits an $\ibp$, since a biclique of $\ibpset$ can
be a single edge of $\graph$. An $\ibp$ becomes interesting when the size of $\ibpset$ is small, say linear in $n$. To give an example, the clique $K_n$
admits $\ibpset=\{\bc{\interval{1}{1}}{\interval{2}{n}},\bc{\interval{2}{2}}{\interval{3}{n}},\bc{\interval{3}{3}}{\interval{4}{n}}, \ldots ,\bc{\interval{n-1}{n-1}}{\interval{n}{n}} \}$ as the interval biclique partition. The set $\ibpset$ gives a
$4 \lceil \log n \rceil |\ibpset|$-bits representation of the graph. 

\begin{lemma}[Lemma 21 in \cite{tww3}]\label{lem:biclpart}
Every $n$-vertex graph $\graph$ with $\tww{\graph} \leq d$ has an interval biclique partition $\ibpset$ of
size at most $(d+1)(n+1)$. Furthermore $\ibpset$ can be computed in time $\bigo{dn}$ given
the ordered union tree of a $d$-sequence for $\graph$. 
\end{lemma}

Lemma~\ref{lem:biclpart} is crucial to our work. Observe that $\ibp$ of a $d$-collapsible graph $\graph$ given by Lemma~\ref{lem:biclpart} assumes an ordering on $V(\graph)$. This ordering is precisely $<_{\tree,\arr}$ given by the ordered union tree $(\tree,\arr)$ required by the statement of Lemma~\ref{lem:biclpart}. So the ordering assumed by $\ibp$ is a twin-width ordering of $\graph$.
In this paper we work with graphs of bounded twin-width and we assume that the appropriate $\ibp$ is at our hand. To conclude this part, we introduce the adjacency matrix for a graph of bounded twin-width, based on its $\ibp$. Let us refer to the vertex ordering assumed by the $\ibp$ as an $\ibp$-ordering.

\begin{definition}\label{def:ibpmatrix}
Let $\graph$ be a graph and assume that $\tww{\graph} \leq d$. 
Let $\ibp$ be its interval biclique partition given by Lemma~\ref{lem:biclpart}. We define $\matibp=\matibpof{\graph}$ as the $0,1$-adjacency matrix of $\graph$ where both rows and columns are ordered according to $\ibp$-ordering.
\end{definition}

Observe, that the set of bicliques $\ibpset$ of $\ibp$ is in fact a set of disjoint rectangles. We can assume that for each biclique $\bc{\interval{i_1}{i_2}}{\interval{j_1}{j_2}} \in \ibpset$ it holds that $i_1 \leq i_2 < j_1 \leq j_2$.  The area determined by the $1$-entries of $\matibp$ above the diagonal is partitioned into $\bigo{dn}$ rectangles $\bc{A}{B} \in \ibpset$. Similarly, the area determined by $1$-entries below the diagonal is partitioned into their reflections $\bc{B}{A}$ for each $\bc{A}{B}\in \ibpset$. To sum up, the entire area determined by $1$-entries of $\matibp$ is partitioned into $\bigo{dn}$ disjoint rectangles with coordinates in $\range{n}$. We denote this set of rectangles as $\rect{\graph}{\ibp}$.

Finally, we move on to defining the twin-width of $0,1$-matrices and introducing crucial properties.
\begin{definition}
Given a~matrix $\matrixx$ and an~integer $\matt$, we define a \emph{$\matt$-division} of $\matrixx$ as the partition of $\matrixx$ into $\matt^2$ rectangular zones.
The zones are obtained in the following way. Rows and columns are partitioned into $\matt$ blocks of (consecutive) rows ($R_1, \ldots R_t$) and (consecutive) columns ($C_1 \ldots C_t$). An intersection of $R_i$ with $C_j$, for $i,j \in \range{t}$, is a zone of $\matt$-division.
\end{definition}
\begin{definition}
Given a $0,1$-matrix $\matrixx$, a $\matt$-grid minor of $\matrixx$ is a $\matt$-division of $\matrixx$ where each zone contains a $1$ entry. A matrix $\matrixx$ is $\matt$-grid free if it has no $\matt$-grid minor. 
\end{definition}
The following theorem lies at the foundation of the whole concept of twin-width.

\begin{theorem}[after \cite{MarcusTardos}]
For every integer $t$, there is some $c_t$ such that every $n \times m$ $0,1$-matrix
$M$ with at least $c_t \max(n,m)$ entries $1$ has a $t$-grid minor. 
\end{theorem}

Cibulka and Kyn\v{c}l \cite{cibulka2019better} decreased $c_t$ down to $\frac{8}{3}(t + 1)^2 2^{4t}$.

\begin{definition}
\label{def:matrix-types}
A matrix is vertical if all its columns are equal, and it is horizontal if all its rows are equal. A matrix is constant if it is both horizontal and vertical. A matrix is mixed, if it is neither horizontal nor vertical.
\end{definition}

\begin{definition}
A $\matt$-mixed minor of a matrix $\matrixx$ is a $\matt$-division of $\matrixx$ where each zone is mixed. If a matrix has no such $\matt$-division, it is called $\matt$-mixed free.   
\end{definition}

We arrive at the theorem that is the heart of \cite{tww1}, which unfortunately uses the twin width of a matrix and the twin-order of a matrix. Due to space limitations, we skip the definitions of the twin-width and the twin-order of a matrix, since they are not crucial for this work. The only claim we need related to these definitions is the following.
\begin{claim}\label{cl:ibp_twword}
For a graph $\graph$ with $\tww{G} \leq d$, the matrix $\matibpof{\graph}$ given by Definition~\ref{def:ibpmatrix} is $d$-twin width ordered. 
\end{claim}
Claim \ref{cl:ibp_twword} can be considered folklore, although there is no formal lemma in \cite{tww1} to provide a citation. Claim \ref{cl:ibp_twword} is further used in combination with the following theorem, which is the main result in \cite{tww1}. We only use the first bullet of this theorem.

\begin{theorem}[after \cite{tww1}] Let $c_t=\frac{8}{3}(t + 1)^2 2^{4t}$.
\label{thm:twin_width_is_mixed_free}
\begin{itemize}
 \item Every $t$-twin-ordered matrix is $(2t+2)$-mixed free.
 \item Every $t$-mixed free matrix has twin-width at most $4 c_t 2^{4 c_t+2} = 2^{2^{O(t)}}$.
\end{itemize}
 
\end{theorem}

